Linearization Algorithms for Fully Composite Optimization

This paper studies first-order algorithms for solving fully composite optimization problems over convex and compact sets. We leverage the structure of the objective by handling its differentiable and non-differentiable components separately, linearizing only the smooth parts. This provides us with new generalizations of the classical Frank-Wolfe method and the Conditional Gradient Sliding algorithm, that cater to a subclass of non-differentiable problems. Our algorithms rely on a stronger version of the linear minimization oracle, which can be efficiently implemented in several practical applications. We provide the basic version of our method with an affine-invariant analysis and prove global convergence rates for both convex and non-convex objectives. Furthermore, in the convex case, we propose an accelerated method with correspondingly improved complexity. Finally, we provide illustrative experiments to support our theoretical results.

==> 00_local_macros.tex <==
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\newcommand{\xpreopt}{x}
\newcommand{\ypreopt}{y}
\newcommand{\filtration}{\mathcal{F}}
\newcommand{\xopt}{x^*}
\newcommand{\yopt}{y^*}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\diam}{\mathcal{D}_{\X}}
\newcommand{\fopt}{f^*}
\newcommand{\f}[1]{f(#1)}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\gradf}{\nabla f}
\newcommand{\lf}{L_f}
\DeclareMathOperator{\Prb}{\mathbb{P}}
\DeclareMathOperator{\prox}{prox}

\newcommand{\norm}[1]{\left\lVert \, #1 \, \right\rVert}
\newcommand{\abs}[1]{\left\lvert \, #1 \, \right\rvert}
\newcommand{\normsqr}[1]{\norm{#1}^2}
\newcommand{\dotprod}[2]{\langle #1 ,\: #2  \rangle}
\newcommand{\bigO}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\bigOtilde}[1]{\mathcal{\Tilde{O}}\left(#1\right)}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\reals}[1]{\mathbb{R}^#1}
\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbb{I}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\Argmax}{Arg\,max}
\DeclareMathOperator{\Argmin}{Arg\,min}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\innerp{\langle}{\rangle}

\allowdisplaybreaks

\def\nn{{ \nonumber }}

\DeclareMathAlphabet{\mathcalorigin}{OMS}{cmsy}{m}{n}
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}

\newtheorem{lemma}{Lemma}
\numberwithin{lemma}{section}

\newtheorem{remark}{Remark}
\numberwithin{remark}{section}

\newtheorem{corollary}{Corollary}
\numberwithin{corollary}{section}

\newtheorem{definition}{Definition}
\numberwithin{definition}{section}

\newtheorem{assumption}{Assumption}
\numberwithin{assumption}{section}

\declaretheorem[name=Theorem,numberwithin=section]{thm-rest}
\declaretheorem[name=Lemma,numberwithin=section]{lem-rest}
\declaretheorem[name=Corollary,numberwithin=section]{cor-rest}
\declaretheorem[name=Definition,numberwithin=section]{def-rest}
\declaretheorem[name=Proposition,numberwithin=section]{prop-rest}
\declaretheorem[name=Assumption,numberwithin=section]{ass-rest}


\allowdisplaybreaks
\def\nn{{ \nonumber }}
\DeclareMathAlphabet{\mathcalorigin}{OMS}{cmsy}{m}{n}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\usepackage[colorinlistoftodos,prependcaption,backgroundcolor=black!5!white,bordercolor=red]{todonotes}

\newcommand{\tr}{\top}
\newcommand{\n}[1]{\|#1 \|}
\newcommand{\lr}[1]{\left\langle #1\right\rangle}

\newcommand{\maria}[1]{ \begin{tcolorbox}[left=2pt, right=2pt, top=2pt, bottom=2pt, boxrule=0.5pt, colback=-red!75!green!70!blue!15!black, colframe=-red!75!green!40!blue!45!]
\textbf{Maria:} #1
\end{tcolorbox}}

\definecolor{mygray}{gray}{0.6}
\newcommand{\eqcomm}[1]{\textcolor{mygray}{[#1]}}


\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\ba{\begin{array}}
\def\ea{\end{array}}
\def\la{\langle}
\def\ra{\rangle}
\def\Def{\stackrel{\mathrm{def}}{=}}

\def\BT{\begin{theorem}}
	\def\ET{\end{theorem}}
\def\BL{\begin{lemma}}
	\def\EL{\end{lemma}}
\def\BC{\begin{corollary}}
	\def\EC{\end{corollary}}
\def\BE{\begin{example}}
	\def\EE{\end{example}}
\def\BD{\begin{definition}}
	\def\ED{\end{definition}}
\def\BR{\begin{remark}}
	\def\ER{\end{remark}}
\def\BAS{\begin{assumption}}
	\def\EAS{\end{assumption}}
\def\BI{\begin{itemize}}
	\def\EI{\end{itemize}}
\def\BP{\begin{proposition}}
	\def\EP{\end{proposition}}


==> 00_packages.tex <==
\usepackage{amssymb,amsmath,amsthm, mathtools}
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{dblfloatfix}
\usepackage{float}
\usepackage[makeroom]{cancel}
\usepackage{subfigure}
\theoremstyle{plain}
\usepackage[colorlinks=true,allcolors=blue]{hyperref}
\usepackage{makecell}
\usepackage{bm}
\usepackage{thm-restate}



==> 2_assumptions_old.tex <==

\section{Setting and Assumptions}
\label{SectionAssumptions}
The problem addressed in this work assumes the following structure on the objective
\beq \label{MainProblem}
\ba{rcl}
\varphi^{\star} & = & \min\limits_{\xx \in \X} 
\Bigl[\,
\varphi(\xx) \;\; \Def \;\;  F( \ff(\xx), \xx)
\,
\Bigr], \qquad \X \subset \R^d,
\ea
\eeq
where $\X$ is a convex and compact set. The inner objective function $\ff: \X \to \R^n$ is differentiable. We write it more precisely as
\beq \label{f_components}
\ba{rcl}
\ff(\xx) & = & (f_1(\xx), \ldots, f_n(\xx)) \;\; \in \;\; \R^n,
\ea
\eeq
where each $f_i: \X \to \R$ is differentiable. Our methods assume access to a first-order oracle for $\ff$.


The outer component $F: \R^n \times \X \to \R$, on the other hand, has a plain and concise representation which is \emph{directly available} to the algorithm designer. The function $F$ is therefore \emph{simple} (a precise meaning is given shortly) but possibly non-differentiable.  

In this work, we propose two algorithmic solutions for solving general problems of type \eqref{MainProblem}, which we call Fully Composite Problems. Our methods importantly rely on efficiently solving linearized subproblems of the following form
\beq \label{MainSubproblem}
\ba{rcl}
\Argmin\limits_{\xx \in \X} F\bigl( \mat{A} \xx + \bb, \xx \bigr)
+ \la \uu, \xx \ra,
\ea
\eeq
where $\mat{A} \in \R^{n \times d}$ and $\bb \in \R^n, \uu \in \R^d$. The algorithms rely on sequential calls to oracles of type~\eqref{MainSubproblem}, whose components are given by the linearizations of the difficult nonlinear functions. When $F$ is the identity mapping, we recover the Linear Minimization Oracle (LMO) used in FW algorithms. Naturally, solving~\eqref{MainSubproblem} is viable only when $F$ is simple and $\X$ has an amenable structure. 



\paragraph{Assumptions.}
We now formally state our main assumptions on the components of the fully composite problem~\eqref{MainProblem}.

\begin{assumption} \label{AssumptionF}
	The outer function $F(\uu, \xx): \R^n \times \X \to \R$ is jointly convex in $\uu$ and $\xx$. Additionally,  $F(\uu, \xx)$ is subhomogeneous in $\uu$:\vspace{-1mm}
	\beq \label{FSubH}
	\ba{rcl}
	F( \gamma \uu, \xx) & \leq & \gamma F(\uu, \xx), 
	\qquad
	\forall \uu \in \R^n, \; \xx \in \X, \; \gamma \geq 1.
	\ea
	\eeq
\end{assumption}

\edef\oldassumption{\the\numexpr\value{assumption}+1}
\setcounter{assumption}{0}
\renewcommand{\theassumption}{\oldassumption\alph{assumption}}

\begin{assumption} \label{AssumptionSmooth}
	The inner mapping $\ff$ is differentiable and the following affine-invariant quantity is bounded:\vspace{-1mm}
	\beq \label{SDef}
	\ba{rcl}
	\mathcal{S} & \!\! = \!\! & \mathcal{S}_{\ff, F, \X}
	\; \Def 
	
	\sup\limits_{\substack{\xx, \yy \in \X, \,\gamma \in (0, 1] \\
			\yy_{\gamma}  = \xx + \gamma(\yy - \xx)}} 
	F\bigl( \frac{2}{\gamma^2}
	\bigl[ \ff(\yy_{\gamma}) - \ff(\xx) - \nabla \ff(\xx)(\yy_{\gamma} - \xx)  \bigr]
	, \yy_{\gamma} \bigr)
	\; < \; +\infty.
	\ea
	\eeq
\end{assumption}

\begin{assumption}\label{AssumptionLipCont} Each component $f_i(\cdot)$
	has a Lipschitz continuous gradient on $\X$ with constant $L_i$. Thus,
	for $1 \leq i \leq n$\vspace{-1mm}
	\begin{equation*}
		\norm{\nabla f_i(\xx) - \nabla f_i(\yy)} \leq L_i \norm{\xx - \yy} \quad \forall \xx, \yy \in \X, 
	\end{equation*}
	and we form the vector of Lipschitz constants: $\mat{L} = (L_1, \ldots, L_n) \in \R^n$.
\end{assumption}
\let\theassumption\origtheassumption

\begin{assumption} \label{AssumptionConvexity}
	Each component $f_i : \X \to \R$ is a convex function.
	Moreover, for any $\xx \in \X$, the function
	$F(\cdot, \xx)$ is monotone. Thus, for any two vectors
	$\uu, \vv \in \R^n$ such that
	$\uu \leq \vv$ (component-wise), it holds that\vspace{-1mm}
	\beq \label{FMonotone}
	\ba{rcl}
	F(\uu, \xx) & \leq & F(\vv, \xx).
	\ea
	\eeq	
\end{assumption}
Assumption~\ref{AssumptionF} represents the formal manner in which we ask that $F$ be simple -- specifically, convexity and bounded growth in the first component. The reader may keep in mind as running examples $F(\uu, \xx) \equiv \max_{i} u^{(i)}$ and	$F(\uu, \xx) \equiv  \| \uu \|$ for an arbitrary fixed norm $\| \cdot \|$. A comprehensive list of examples and applications satisfying Assumption~\ref{AssumptionF} is given in Section~\ref{SectionApplications}.


For mappings $\ff$ that are twice differentiable, we can bound the quantity $\mathcal{S}$
from Assumption~\ref{AssumptionSmooth} using Taylor's formula
and the second derivatives, as follows
$$
\ba{rcl}
\mathcal{S} & \leq & 
\sup\limits_{\substack{\xx, \yy \in \X, \, \gamma \in [0, 1] \\
		\yy_{\gamma}  = \xx + \gamma(\yy - \xx)}}
F( \nabla^2 \ff(\yy_{\gamma})[\yy - \xx]^2, \xx ).
\ea
$$
This quantity is reminiscent of the quadratic upper-bound used to analyze smooth optimization methods.
In particular, for the common setting of compactness of $\X$
and Lipschitz continuity of $\nabla f_i$ with respect to a fixed norm $\| \cdot \|$, the assumption is satisfied with
$$
\ba{rcl}
\mathcal{S} & \leq & F(\mat{L} \diam^2 ) \;\; \Def \;\; \sup\limits_{\xx \in \X} F(\mat{L} \diam^2, \xx ),
\ea
$$
where $\diam$ is the diameter of $\X$,
and $\mat{L}$ is the vector of Lipschitz constants. Note that in its present formulation, Assumption~\ref{AssumptionSmooth} is \textit{affine-invariant} and hence does not depend on a particular choice of the norm. The importance of affine-invariant characterizations of the classical FW algorithm is discussed by \citet{jaggi2013revisiting}.
Moreover, Assumption~\ref{AssumptionSmooth} implies global progress bounds for our fully composite objective with an inner linearization of $\ff$, as stated in the following Lemma~\ref{LemGlobalBounds}. The proof is straightforward and deferred to the appendix.
\begin{restatable}{lem-rest}{LemGlobalBounds}
	\label{LemGlobalBounds}
	Let $\xx, \yy \in \X$ and $\gamma \in [0, 1]$.
	Denote $\yy_{\gamma} = \xx + \gamma(\yy - \xx)$.
	Then, it holds
	\beq \label{PhiContrBound}
	\ba{rcl}
	\varphi(\yy_{\gamma}) & \leq & 
	F\bigl( \ff(x) + \nabla \ff(\xx)(\yy_{\gamma} - \xx), \, \yy_{\gamma}  \bigr)
	\; + \;
	\frac{\gamma^2}{2} \mathcal{S}.
	\ea
	\eeq
\end{restatable}
Assumption~\ref{AssumptionLipCont} is standard in the literature and considered separately from Assumption~\ref{AssumptionSmooth} to allow for different levels of generality in our results. Note that the functions need only be $L_i$-smooth on the convex and compact set $\X$ and hence this requirement is actually a locally-Lipschitz gradient assumption on the functions $f_i$.


Finally, Assumption~\ref{AssumptionConvexity} is used for deriving improved convergence guarantees for the case in which the mapping $\ff$ is convex. Given that objective~\eqref{MainProblem} is a composition of $F$ and $\ff$, assuming convexity of each component separately is not sufficient to ensure an overall convex problem, and an additional \emph{monotonicity} condition is required \citep[see][]{boyd2004convex}. Since it is a further specification on $F$, the set of conforming examples is reduced (e.g., norms are not monotone, but max-type minimization still satisfies this assumption. See Section~\ref{SectionApplications}). The combination of Assumptions~\ref{AssumptionF} and \ref{AssumptionConvexity} leads to the convexity of objective \eqref{MainProblem} and enables us to achieve asymptotically faster convergence rates. 

==> 6_experiments_old.tex <==
\section{Applications}
\label{SectionApplications}


We start by demonstrating how the standard problem formulations of  Frank-Wolfe algorithms and Proximal Gradient schemes can be derived from our problem template.
\begin{example} \label{ExampleFW}
	Let $F(\uu, \xx) \equiv u^{(1)}$. Then, problem \eqref{MainProblem} reduces to $\displaystyle	\min\limits_{\xx \in \X} f_1(\xx).$ Consequently, subproblem \eqref{MainSubproblem} reduces to the LMO used in CG methods: $\displaystyle \argmin\limits_{\xx \in \X} \la \uu, \xx \ra$.
\end{example}
\begin{example}
	Let $F(\uu, \xx) \equiv u^{(1)} + \psi(\xx)$, where $\psi$ is a given convex function (e.g., a simple regularizer).
	Then, problem~\eqref{MainProblem} reduces to additive composite optimization~\citep{nesterov2013gradient,beck2009fast} $\displaystyle 	\min\limits_{\xx \in \X} \Bigl\{  f_1(\xx) + \psi(\xx) \Bigr\},$
	and subproblem \eqref{MainSubproblem} becomes $\displaystyle	\argmin\limits_{\xx \in \X} \Bigl\{  \la \uu, \xx \ra + \psi(\xx) \Bigr\}.$
\end{example}
We further provide interesting practical settings that can be modeled through our fully composite template and for which $F$ satisfies Assumption~\ref{AssumptionF}. Additional examples are included in the appendix.

\begin{example} \label{ExampleMax}
	Let $F(\uu, \xx) \equiv \max\limits_{1 \leq i \leq n} u^{(i)}$, which conforms to Assumptions~\ref{AssumptionF}~and~\ref{AssumptionConvexity}.
	Then, problem \eqref{MainProblem} is the max-type minimization:
	\beq \label{MinMax}
	\ba{c}
	\min\limits_{\xx \in \X} \max\limits_{1 \leq i \leq n} f_i(\xx),
	\ea
	\eeq
	and the subproblem is
	\beq \label{MaxSubproblem}
	\ba{rcl}
	\min\limits_{\xx \in \X} \max\limits_{1 \leq i \leq n} \la \aa_i, \xx \ra + b_i
	& \quad \Leftrightarrow \quad &
	\min\limits_{\xx \in \X, t \in \R} \bigl\{ t \; : \; \la \aa_i, \xx \ra + b_i \leq t, \, 1 \leq i \leq n \bigr\}.
	\ea
	\eeq
	Note that if $\X$ is a polyhedron, then this problem is an instance of Linear Programming.
	In case of general $\X$, we can apply Interior-Point Methods~\citep{nesterov1994interior}.
	Another option for solving subproblems \eqref{MaxSubproblem} is to use duality.
	Denoting the standard simplex by $\Delta_n \Def \{ \blambda \in \R^{n}_{+} \, : \, \la \blambda, \ee \ra = 1 \}$,
	where $\ee$ is the vector of all ones and under strong duality~\citep{rockafellar1970convex} we have
	\beq \label{MaxTypeSubproblem}
	\ba{rcl}
	\min\limits_{\xx \in \X} \max\limits_{1 \leq i \leq n} \la \aa_i, \xx \ra + b_i
	& = & 
	\min\limits_{\xx \in \X} \max\limits_{\blambda \in \Delta_n}
	\sum\limits_{i = 1}^n \lambda^{(i)} \bigl[  \la \aa_i, \xx \ra + b_i \bigr]  = 
	\max\limits_{\blambda \in \Delta_n} g(\blambda),
	\ea
	\eeq
	where $g(\blambda) \Def \min\limits_{\xx \in \X} \sum_{i = 1}^n \lambda^{(i)} \bigl[  \la \aa_i, \xx \ra + b_i \bigr] $.
	Thus, our subproblem becomes
	the maximization of a concave function $g(\blambda)$ over the simplex.
	It can be done very efficiently for small values of $n$ (by using, e.g. the Ellipsoid Method or
	the Mirror Descent algorithm).	Computing the value and the subgradient of $g(\blambda)$ reduces to just one call of LMO for $\X$.
	
	Problems of this type are common in applications
	with \emph{Multi-objective Optimization}.
	Using max-type scalarization like in \eqref{MinMax},
	leads to the \emph{Pareto front} convergence
	for multi-objective problems~\citep{zhang2020random}.
	An interesting case is $n = 2$, which leads to
	$
	\ba{rcl}
	\min\limits_{\xx \in \X} \max \bigl\{ f_1(\xx), f_2(\xx) \bigr\}.
	\ea
	$
	The corresponding subproblem is then 
	a \emph{univariate} maximization of a concave function:
	$$
	\ba{rcl}
	\max\limits_{\lambda \in [0, 1]}
	g(\lambda) ,
	\qquad \text{with} \qquad
	g(\lambda) & \Def & \min\limits_{\xx \in \X}
	\Bigl\{ \lambda \bigl[  \la \aa_1, \xx \ra + b_1  \bigr]
	+ (1 - \lambda) \bigl[ \la \aa_2, \xx \ra + b_2  \bigr]
	\Bigr\}.
	\ea
	$$
	One may use binary search to solve it, requiring only a logarithmic number of LMOs over $\X$. 
\end{example}

\begin{example} \label{ExampleNorm}
	Let
	$
	F(\uu, \xx) \equiv  \| \uu \| 
	$
	for an arbitrary fixed norm $\| \cdot \|$, which satisfies Assumption~\ref{AssumptionF}. Then, problem~\eqref{MainProblem}
	can be interpreted as solving a system of non-linear equations
	over $\X$:
	\beq \label{GSProblem}
	\ba{rcl}
	\min\limits_{\xx \in \X} \| \ff (\xx) \|,
	\ea
	\eeq
	and the subproblem is solving the (constrained) linear system 
	$
	\min\limits_{\xx \in \X} \| \mat{A}\xx + \bb \|	$. Problems of these kind can be encountered in applications such as constrained robust phase retrieval~\citep{duchi2019solving}.
	Then, the iterations of Algorithm~\ref{alg:basic} can be interpreted as a variant
	of the \textit{Gauss-Newton method},
	solving the (constrained) linear systems:
	\beq \label{GSAlgEx}
	\xx_{k + 1}  \in  \Argmin\limits_{\xx \in \X}
	\| \ff(\yy_k) + \nabla \ff(\yy_k)(\xx - \yy_k) \|, \ \ \text{ and }\ \ 
	\yy_{k + 1}  =  (1 - \gamma_k) \yy_k + \gamma_k \xx_{k + 1}.
	\eeq
	Depending on the norm choice, we can impose different properties on the solution, such
	as sparsity.
\end{example}
When solving problem~\eqref{GSProblem}, the accuracy measure $\Delta_k$ defined in Section~\ref{SectionBasic} can be meaningfully interpreted. For example, we consider the Euclidean norm,
and denote the squared objective by
$\Phi(\xx) \Def \frac{1}{2}\bigl[ \varphi(\xx) \bigr]^2 = \frac{1}{2} \| \ff(\xx) \|^2$.
Then the accuracy measure $\Delta_k$ is related to the classical FW gap for the squared loss. We can therefore prove the following global convergence result, 
which is a direct consequence from our theory in Section~\ref{SectionBasic}. The proof is deferred to the appendix.

\begin{restatable}{prop-rest}{PropNorm}\label{PropNorm}
	Let $\gamma_k := \frac{1}{\sqrt{1 + k}}$. Then, 
	for the iterations \eqref{GSAlgEx}, we have
	$$
	\ba{rcl}
	\min\limits_{0 \leq i \leq k}
	\max\limits_{\yy \in \X }\la \nabla \Phi(\yy_k), \yy_k - \yy \ra
	& \leq & 
	\cO\bigl(\frac{\ln (k + 1)}{k}\bigr), \quad k \geq 1.
	\ea
	$$	
\end{restatable}



\vspace{-4mm}
\section{Experiments}
\label{SectionExperiments}
\begin{figure*}[t!]
	\centering
	\begin{minipage}[t]{\textwidth}
		\setlength{\lineskip}{0pt}
		\subfigure[]{
			\centering
			\includegraphics[width=.44\linewidth]{../figures/results_simplex_dim=500,FOcalls}
			\label{FigSimplexFO}
		}\hspace{5mm}
		\subfigure[]{
			\centering
			\includegraphics[width=.44\linewidth]{../figures/results_simplex_dim=500,SubproblemOraclecalls}
			\label{FigSimplexLMO}
		}
		\vspace{-3mm}
		\caption{Convergence of the Basic and Accelerated methods against the Projected Subgradient baseline and the relevant theoretical rates.} 
		\vspace{-2mm}
	\end{minipage}
\end{figure*}
We provide experiments in two different problem settings, one of which is deferred to the appendix, %
along with other experimental details such as data generation and hyperparameter settings. For both experiments we use the projected subgradient method with decreasing stepsize~\citep{shor2012minimization} as a baseline, and the \texttt{CVXPY} library \citep{diamond2016cvxpy} to solve the subproblems of type~\eqref{MainSubproblem}.

\vspace{-1mm}
\paragraph{Minimization over the simplex.} We consider the following optimization problem:
\begin{align}
	\min_{\xx \in \X}\left\{ \max_{i = 1, n} \xx^\top \AA_i \xx  - \bb_i^\top\xx \right\}, \text{ for } \X = \Delta_d \subseteq \R^d\nn,
\end{align}
where $ \AA_i \in \R^{d \times d}$ are random PSD matrices and $\bb \in \R^d$. We use $d = 500$ and $n = 10$. The convergence results in terms of FO oracles and oracles of type~\eqref{MainSubproblem} are shown in Figure~\ref{FigSimplexFO}~and~\ref{FigSimplexLMO}, respectively. The figure highlights the improvement in terms of the number of FO calls, while showing comparable performance in terms of subproblem oracle calls, as predicted by our theory. 
\vspace{-2mm}
\section{Conclusion} Our work illustrates how, by assuming additional structure within a class of objectives (e.g., non-differentiable ones), improved convergence rates may be attained. Moreover, it shows how a simple principle, such as linearizing the differentiable components of a function composition, can be used to create more benign subproblems that are efficiently solved. Interesting future work can address relaxing the assumptions on $F$ and extending this framework to stochastic settings.

